Finite-size Effects in periodic EOM-CCSD for Ionization Energies and Electron Affinities: Convergence Rate and Extrapolation to the Thermodynamic Limit

We investigate the convergence of quasi-particle energies for periodic systems to the thermodynamic limit using increasingly large simulation cells corresponding to increasingly dense integration meshes in reciprocal space. The quasi-particle energies are computed at the level of equation-of-motion coupled-cluster theory for ionization (IP-EOM-CC) and electron attachment processes (EA-EOM-CC). By introducing an electronic correlation structure factor, the expected asymptotic convergence rates for systems with different dimensionality are formally derived. We rigorously test these derivations through numerical simulations for trans-Polyacetylene using IP/EA-EOM-CCSD and the G0W0@HF approximation, which confirm the predicted convergence behavior. Our findings provide a solid foundation for efficient schemes to correct finite-size errors in IP/EA-EOM-CCSD calculations.

==> Makefile <==
figdi = $(PWD)/figures

all: main.pdf

clean:
	latexmk -C

.PHONY: clean all

# pure_cut_coulomb_general_finite_size_convergence_compare_fits.pdf
# pure_cut_coulomb_general_finite_size_convergence_compare_leading_orders.pdf
# pure_cut_coulomb_general_finite_size_convergence_eom_vs_gw.pdf
# pure_cut_coulomb_general_finite_size_convergence.pdf
# pure_cut_coulomb_general_gw_finite_size_convergence.pdf
#


fig_lih = \
$(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_EA.pdf \
$(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_GAP.pdf \
$(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_IP.pdf

$(fig_lih): ./data/scripts/LiH-SFs/plot_rad_sf_10_vs_50_vs_100_small_G.py
	cd ./data/scripts/LiH-SFs/; python3 plot_rad_sf_10_vs_50_vs_100_small_G.py
	cd ./data/scripts/LiH-SFs/; mv -v rad_* $(figdi)/

FIGURES += $(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_IP_EA_GAP.pdf
$(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_IP_EA_GAP.pdf: ./data/scripts/LiH-SFs/plot_rad_sf_10_vs_50_vs_100_small_G_all_in_one.py
	cd ./data/scripts/LiH-SFs/; python3 plot_rad_sf_10_vs_50_vs_100_small_G_all_in_one.py
	cd ./data/scripts/LiH-SFs/; mv -v rad_* $(figdi)/

FIGURES += $(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_ground_state.pdf
$(figdi)/rad_avg_structure_factor_smallG_10_vs_50_vs_100_ground_state.pdf: ./data/scripts/LiH-SFs/plot_rad_ground_state_sf_10_vs_50_vs_100_small_G_all_in_one.py
	cd ./data/scripts/LiH-SFs/; python3 plot_rad_ground_state_sf_10_vs_50_vs_100_small_G_all_in_one.py
	cd ./data/scripts/LiH-SFs/; mv -v rad_* $(figdi)/

FIGURES += $(figdi)/pure_cut_coulomb_general_downsampledfinite_size_convergence_compare_leading_orders_oaf_1e3_all_nk.pdf
$(figdi)/pure_cut_coulomb_general_downsampledfinite_size_convergence_compare_leading_orders_oaf_1e3_all_nk.pdf: ./data/scripts/eom-downsampled/determine_general_downsampled_finite_size_extrapolation_law_leading_orders_oaf_1e3_all_nk.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv pure* $(figdi)


FIGURES += $(figdi)/pure_cut_coulomb_general_downsampled_finite_size_convergence_eom_oaf_1e3_vs_drccd_eom_all_nk.pdf
$(figdi)/pure_cut_coulomb_general_downsampled_finite_size_convergence_eom_oaf_1e3_vs_drccd_eom_all_nk.pdf: ./data/scripts/eom-vs-drccd-downsampled/plot_eom_oaf_1e3_vs_drccd_eom_downsampled_all_nk.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv pure* $(figdi)

FIGURES += $(figdi)/pure_cut_coulomb_general_downsampled_finite_size_convergence_eom_oaf_1e3_vs_gw_all_nk.pdf
$(figdi)/pure_cut_coulomb_general_downsampled_finite_size_convergence_eom_oaf_1e3_vs_gw_all_nk.pdf: ./data/scripts/eom-vs-gw-downsampled/plot_eom_oaf_1e3_vs_gw_downsampled_all_nk.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv *pdf *png $(figdi)

FIGURES += $(figdi)/pure_cut_coulomb_general_finite_size_convergence_compare_leading_orders_oaf_1e3_all_nk.pdf
$(figdi)/pure_cut_coulomb_general_finite_size_convergence_compare_leading_orders_oaf_1e3_all_nk.pdf: ./data/scripts/eom/determine_general_finite_size_extrapolation_law_leading_orders_oaf_1e3_all_nk.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv *pdf *png $(figdi)

FIGURES += $(figdi)/pure_cut_coulomb_general_finite_size_convergence_eom_oaf_1e3_vs_gw_all_nk.pdf
$(figdi)/pure_cut_coulomb_general_finite_size_convergence_eom_oaf_1e3_vs_gw_all_nk.pdf: ./data/scripts/eom-vs-gw/plot_eom_vs_gw_oaf_1e3_all_nk.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv *pdf *png $(figdi)

FIGURES += $(figdi)/1d_along_z_structure_factor_smallG_1x1x32_tpa_EA_IP_GAP_mirrored.pdf
$(figdi)/1d_along_z_structure_factor_smallG_1x1x32_tpa_EA_IP_GAP_mirrored.pdf: ./data/scripts/tPA-SFs/plot_1d_along_z_ea_ip_gap_mirrored.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv *pdf *png $(figdi)

FIGURES += $(figdi)/finite_size_convergence_tPA3_no_downsampling_3Z.pdf
$(figdi)/finite_size_convergence_tPA3_no_downsampling_3Z.pdf: ./data/scripts/eom-tpa3/determine_general_finite_size_extrapolation_law_leading_orders_oaf_1e3_all_nk_tPA3.py
	cd $(<D); python3 $(notdir $<)
	cd $(<D); mv *pdf *png $(figdi)



# todremove
# pure_cut_coulomb_general_downsampledfinite_size_convergence_compare_leading_orders.pdf
# pure_cut_coulomb_general_downsampled_finite_size_convergence_eom_vs_gw.pdf

FIGURES += \
$(fig_lih) \

main.pdf: main.tex $(FIGURES)
	latexmk -pdf -synctex=1 -shell-escape main.tex


